Vulnerability Analysis of Nonlinear Control Systems to Stealthy False Data Injection Attacks

In this work, we focus on analyzing vulnerability of nonlinear dynamical control systems to stealthy false data injection attacks on sensors. We start by defining the stealthiness notion in the most general form where an attack is considered stealthy if it would be undetected by any intrusion detector, i.e., any intrusion detector could not do better than a random guess. Depending on the level of attacker's knowledge about the plant model, controller, and the system states, two different attack models are considered. For each attack model, we derive the conditions for which the system will be vulnerable to stealthy impactful attacks, in addition to finding a methodology for designing such sequence of false data injection attacks. When the attacker has complete knowledge about the system, we show that if the closed loop system is incrementally exponentially stable while the open loop plant is incrementally unstable, then the system is vulnerable to stealthy yet impactful attacks on sensors. However, in the second attack model, with less knowledge about the system, additional conditions need to be satisfied and the level of stealthiness depends on the accuracy of attacker's knowledge about the system. We also consider the impact of stealthy attacks on state estimation, and show that if the closed loop control system including the estimator is incrementally stable, then the state estimation in the presence of attack converges to the attack free estimates. Finally, we illustrate our results on numerical case studies.

==> Resiliency.tex <==
\section{Resiliency of Nonlinear Systems to Stealthy Attacks} \label{sec:resiliency}

In previous section, we considered the vulnerability of nonlinear control systems and derive the conditions for the existence of impactful yet stealthy attacks. We observed that the instability of the open-loop dynamics helps the attacker to design impactful attacks while IES (or IISS) of the closed-loop control system causes the attack to be stealthy. In contrast, in this section we intend to see what will happen if instead the open-loop system is stable and whether such class of nonlinear control systems can be resilient to stealthy sensor attacks. We will see that achieving resilience for system in form of~\eqref{eq:plant} and~\eqref{eq:control} is not possible in general, however, with slight change in the system's controller we can reach to resilience for a class open-loop stable control systems.

Let assume that there exists a sensor ($i$-th) with measurement value at time $t$ denoted by $y^c_{t,i}$ for which the system and controller satisfy
\begin{equation}\label{eq:state_output}
\lim_{\vert y^c_{t,i} \vert \to \infty} \Vert f\big(x_{t-1},h_c\big(f_c(\mathpzc{X}_{t-1},y_t^c),y_t^c\big)\big) \Vert \to \infty,
\end{equation}
which means for arbitrarily large values of received $i$-th sensor measurement by controller, the states norm will become arbitrarily large. For example, the LTI model in~\eqref{eq:lti} satisfies this property. Now, assume that the attacker chooses to compromise  the $i$-th sensor at only one time step ($t=0$) with measurement value of $y_{0,i}$, and let assume the attack value is denoted  by $a_{0,i}$. Then, the received $i$-th measurement by the controller is $y_{0,i}^{c,a}=y_{0,i}+a_{0,i}$. If the attacker chooses arbitrarily large $a_{0,i}$, the states at time step one will become arbitrarily large according to~\eqref{eq:state_output}. This means the attacker can cause large impact on the states of the system by attacking only at time step zero. On the other hand, since we assume the measurement noise is Gaussian, it is feasible for $v_{0,i}$ to take any value in $\mathbb{R}$. Hence, the ID cannot detect such an attack as a significant increase in measurement within a single time step may also be attributed to Gaussian noise.


Consequently, any system in form of~\eqref{eq:plant} and~\eqref{eq:control} that satisfies~\eqref{eq:state_output} is vulnerable to such one time step attacks. However, in real world physical systems the controllers are designed in a way that such huge jumps in measurements (commonly called as outliers) are rejected (for example, LQG controllers that use $\chi^2$ detectors for outlier detection).  Accordingly, let assume that for each sensor $i$, the received measurement $y_{t,i}^c$ is compared with its nominal value $\bar{y}_{t,i}$ at time $t$ and if $|y_{t,i}^c-\bar{y}_{t,i}|>\eta$ holds for some threshold $\eta$, then such sensor measurement will be rejected by the controller. Under such condition, the controller either uses the sensor measurement that is not rejected or find a predicted value using previous measurements\footnote{It should be noted that the nominal sensor measurements $\bar{y}$ can be obtained either by using Kalman (or Extended Kalman filter) estimates of observation or the system's own knowledge about the range of possible observation (for example by looking at previous measurements).}. Under such condition if we denote the used sensor measurement in the controller by $y^{u}$, then the controller~\eqref{eq:control} can be rewritten in the following form
\begin{equation}
\label{eq:control_res}
\begin{split}
\mathpzc{X}_{t} &= f_c(\mathpzc{X}_{t-1},y_t^u),\\
u_t  &= h_c(\mathpzc{X}_{t},y_t^u),
\end{split}
\end{equation}


for any $t$, where it should satisfy $\Vert y_{t}^u-\bar{y}_{t}\Vert_{\infty}\leq \eta$. 




\begin{theorem}
Assume that the open-loop system~\eqref{eq:input-state} and the controller dynamics~\eqref{eq:control_res} are IISS with functions $\gamma$ and $\gamma_c$ functions in class $\mathcal{K}_{\infty}$, respectively and the function $h_c$ is Lipschitz with constant $L_{h_c}$. Then, the deviation in the states caused by the sensor attack will be limited as $\Vert x_t^a-x_t\Vert\leq \gamma(L_{h_c}(\gamma_c(2\eta)+\eta))$ for all time steps $t\in \mathbb{Z}_{\geq 0}$.
\end{theorem}


\begin{proof}
Consider the dynamics of the controller when the system is attack free and when it is under attack as follows

\begin{equation}
\begin{split}
\mathpzc{X}_{t} &= f_c(\mathpzc{X}_{t-1},y_t^u),\\
\mathpzc{X}_{t}^a &= f_c(\mathpzc{X}_{t-1}^a,y_t^{u,a}).
\end{split}
\end{equation}
Since the above dynamics is IISS we get 
\begin{equation}
\begin{split}
\Vert \mathpzc{X}_{t}^a-\mathpzc{X}_{t}\Vert &\leq  \gamma_c(\Vert y_t^{u,a}-y_t^u\Vert_{\infty})\leq \gamma_c(\Vert y_t^{u,a}-\bar{y}_{t}+\bar{y}_{t}-y_t^u\Vert_{\infty})\\
&\leq \gamma_c(\Vert y_t^{u,a}-\bar{y}_{t} \Vert_{\infty} + \Vert y_t^u -\bar{y}_{t} \Vert_{\infty})\leq \gamma_c(2\eta),
\end{split}
\end{equation}

where we used $\mathpzc{X}_{0}=\mathpzc{X}_{0}^a$, $\Vert y_t^{u,a}-\bar{y}_{t} \Vert_{\infty}\leq \eta$, $\Vert y_t^{u}-\bar{y}_{t} \Vert_{\infty}\leq \eta$, and the fact that $\gamma_c\in \mathcal{K}_{\infty}$ is strictly increasing function. Then, using the Lipschitz property of the function we get 
\begin{equation}
\begin{split}
\Vert u_t^a-u_t\Vert &\leq  \Vert h_c(\mathpzc{X}_{t}^a,y_t^{u,a})-h_c(\mathpzc{X}_{t},y_t^u)\Vert \\
&\leq L_{h_c}(\Vert \mathpzc{X}_{t}^a-\mathpzc{X}_{t}\Vert +\Vert y_t^{u,a}-y_t^u\Vert_{\infty})\\
&\leq L_{h_c}(\gamma_c(2\eta)+\eta)
\end{split}
\end{equation}
Using our assumption that the open-loop system dynamics~\eqref{eq:input-state} are IISS, we have 
\begin{equation}
\begin{split}
\Vert x_{t}^a-x_{t}\Vert &\overset{(i)}{\leq}  \gamma(\Vert U_t^{a}-U_t\Vert_{\infty})\overset{(ii)}{\leq} \gamma(\Vert u_t^{a}-u_t\Vert_{\infty})\\
&\overset{(iii)}{\leq} \gamma(L_{h_c}(\gamma_c(2\eta)+\eta)),
\end{split}
\end{equation}
where we used the fact that $x_0=x_0^a$ in $(i)$, $w_t^a=w_t$ in $(ii)$ and the norm property that 2-norm is always upper bounded by infinity norm in $(iii)$.
\end{proof}


Therefore, if the controller rejects the outlier observations, the open-loop and the controller dynamics are IISS, then the attacker's impact on the states will be limited and cannot be arbitrarily large.

\begin{remark}
It should be noted that even though outlier observation rejection in the controller helped the system to be resilient against general attacks for IISS open-loop dynamics, it will not be effective against stealthy attacks if the open-loop system is  unstable and the closed-loop control system is IES closed-loop. This is because the observation trajectory of under attack system exponentially converges to observation of the attack free system. Therefore, this strategy is ineffective against our proposed attack when the conditions of Theorem~\ref{thm:PAt_1} and~\ref{thm:PA_2} are satisfied.  
\end{remark}




